Optimal Confidence Regions for the Multinomial Parameter

Construction of tight confidence regions and intervals is central to statistical inference and decision making. This paper develops new theory showing minimum average volume confidence regions for categorical data. More precisely, consider an empirical distribution $\widehat{\boldsymbol{p}}$ generated from $n$ iid realizations of a random variable that takes one of $k$ possible values according to an unknown distribution $\boldsymbol{p}$. This is analogous to a single draw from a multinomial distribution. A confidence region is a subset of the probability simplex that depends on $\widehat{\boldsymbol{p}}$ and contains the unknown $\boldsymbol{p}$ with a specified confidence. This paper shows how one can construct minimum average volume confidence regions, answering a long standing question. We also show the optimality of the regions directly translates to optimal confidence intervals of linear functionals such as the mean, implying sample complexity and regret improvements for adaptive machine learning algorithms.

==> general_spaces.tex <==


\subsection{Minimal Confidence Sets for General Measure Spaces}

\textcolor{red}{This paper also extends the aforementioned results to general measure spaces related through a conditional probability measure.  The more general case is presented in \ref{sec:gen}, as the level of abstraction can obscure the importance of the results in the multinomial case.  In addition to confidence regions for the multinomial parameter, we show the general theory reduces to well understood confidence regions for the case of the mean of an i.i.d. Gaussian.} 

The concept of a minimal volume confidence construction extends to general measure spaces related through a conditional probability distribution.  This setting encompasses a number of settings, including well studied problems, such as finding a confidence regions for the  mean of a unit variance Gaussian random variable. 

Consider $\theta \in \Theta$ and $\widehat{\theta} \in \Theta'$ where $\Theta$ and $\Theta'$ are measure spaces equipped with measures $\mu(\cdot)$ and $\nu(\cdot)$ respectively, related through a probability measure over a $\sigma$-algebra on $\Theta'$, $\mathbb{P}( \mathcal{S} | \theta) = \mathbb{P}_{ \theta} ( \mathcal{S} )$.
Denote $\mathcal{P}(\Theta)$ and $\mathcal{P}(\Theta')$ the $\sigma$-algebra on $\Theta$ and $\Theta'$ respectively.
Let  $\mathcal{S({\theta})}: \Theta \rightarrow \mathcal{P}(\Theta')$ be the preimage of $\mathcal{C}_{\delta}( \widehat{\theta})$:
\begin{eqnarray}  
\mathcal{S({\theta})} = \left\{ \widehat{ \theta } \in  \Theta' : \theta \in \mathcal{C}_{\delta}( \widehat{\theta} ) \right\}.
\end{eqnarray}
Then 
\begin{eqnarray} 
\theta \in \mathcal{C}_\delta(\widehat{\theta}) \Leftrightarrow  \widehat{\theta}  \in \mathcal{S}(\theta)
\end{eqnarray}
and 
\begin{eqnarray}
\mathcal{C}_{\delta} (\widehat{\theta}) = \left\{\theta \in \Theta :  \widehat{\theta} \in \mathcal{S}({\theta}) \right\}.
\end{eqnarray}

\begin{defi} \label{def:minvolgeneral}
Minimal volume confidence region.   Let $\mathcal{S^\star({\theta})}: \Theta \rightarrow \mathcal{P}(\Theta')$ be any set valued function that satisfies
\begin{eqnarray} \label{eqn:stheta_min}
\mathcal{S}^\star (\theta) = \arg \min_{\left\{\mathcal{S} \in \mathcal{P}(\Theta') : \mathbb{P}( \mathcal{S} | \theta ) \geq 1-\delta \right\}} \nu(\mathcal{S})
\end{eqnarray}
for all $\theta$. 
%\begin{eqnarray}
%\mathbb{P}_{\theta}(\widehat{\theta}) = \frac{ \int_{\bp: f(\bp)= \theta}  \mathbb{P}_{\bp}( \widehat{\theta} ) d\bp  }{ \int_{\bp: f(\bp)= \theta} d\bp } 
%\end{eqnarray}
The minimal measure confidence region is given as 
\begin{eqnarray} \label{eqn:theta_inv}
\mathcal{C}_{\delta}^\star(\widehat{\theta}) := \left\{\theta \in\Theta :  \widehat{\theta} \in \mathcal{S}^\star({\theta}) \right\}.
\end{eqnarray}
\end{defi}
\noindent
$\mathcal{S}^\star({\theta})$ is a set valued function, mapping  $\theta$ to a subset of $\Theta'$ with minimal measure among subsets whose probability under $\theta$ equals or exceeds $1-\delta$.   $\mathcal{C}_{\delta}^\star(\widehat{\theta})$ is the subset of $\Theta$ for which the set valued function $\mathcal{S}^\star({\theta})$ includes $\widehat{\theta}$.  
\begin{obs}
  $\mathcal{C}_{\delta}^\star(\widehat{\theta})$ is a confidence region at level $1-\delta$ since 
$\mathbb{P}_{\theta}  \left( \theta \in \mathcal{C}^\star_{\delta}( \widehat{\theta}) \right)
=    \mathbb{P}_{\theta} \left( \mathcal{S}^\star (\theta)  \right) \geq 1-  \delta$.
\end{obs}
\begin{thm} \label{thm:general}
Let $\mathcal{C}_{\delta}^\star(\widehat{\theta})$ be a confidence region given by Definition~\ref{def:minvolgeneral}.  Then 
\begin{eqnarray} \nonumber
\int  \mu ( C_{\delta}^\star (\widehat{\theta} )  )   d\nu(\widehat{\theta})  \leq  \int  \mu ( C_{\delta} (\widehat{\theta} )  )   d\nu(\widehat{\theta}) 
\end{eqnarray}
for any confidence region $\mathcal{C}_{\delta}(\widehat{\theta})$.
\end{thm}

\begin{proof}
Proof of Theorem \ref{thm:general} follows in a similar manner as proof of \ref{thm:main}.  First note that 
\begin{eqnarray}
\int  \mu ( C_{\delta} (\widehat{\theta} )  )   d\nu(\widehat{\theta}) =  \int  \nu ( \mathcal{S} (\theta ) ) d\mu ({\theta})  
\end{eqnarray}
since 
\begin{eqnarray*}
\int  \mu ( C_{\delta} (\widehat{\theta} )  )   d \nu(\widehat{\theta}) &=& \int  \int   \mathbbm{1}_{ \{\theta \in \mathcal{C}_{\delta} (\widehat{\theta}) \} } d\mu ({\theta})  d\nu( \widehat{\theta}) \\
&=&\int  \int   \mathbbm{1}_{ \{\theta \in \mathcal{C}_{\delta} (\widehat{\theta}) \} }   d\nu(\widehat{\theta}) d\mu({\theta}) \\
&=&\int  \int   \mathbbm{1}_{ \{\widehat{\theta} \in \mathcal{S}(\theta) \} }   d\nu (\widehat{\theta}) d\mu({\theta})  \\
&=&  {\int \nu( \mathcal{S}( \theta ) ) d\mu(\theta) }.
\end{eqnarray*}
Since $\nu(\mathcal{S}^\star (\theta)) \leq \nu(\mathcal{S} (\theta))$ by definition, this completes the proof.   
\end{proof}

\begin{ex}
Consider $X_1, \dots, X_n \overset{iid}{\sim} \mathcal{N}(\theta,1)$ and let $\widehat{\theta}$ the sample mean. In this cases, $\Theta = \Theta' = \mathbb{R}$ and $\mu(\cdot) = \nu(\cdot)$ is the Lebesgue measure.  Then
\begin{eqnarray*}
\mathcal{S}^\star (\theta) &=& \arg \min_{ \left\{ \mathcal{S} \subset \mathbb{R} : \mathbb{P}( \mathcal{S}| \theta)  \geq 1-\delta \right\} } \mu(\mathcal{S}) \\
&=& \left[\theta - \gamma, \theta + \gamma \right].
\end{eqnarray*}
where $\gamma = \left\{ x: \int_x^{\infty}\frac{1}{\sqrt{2\pi/n}} e^{-n x^2/2} = \delta/2 \right\} $ and 
\begin{eqnarray*}
\mathcal{C}^{\star}_{\delta} (\widehat{\theta}) &=& \left\{\theta \in \Theta :  \widehat{\theta} \in  \left[\theta - \gamma, \theta + \gamma \right]  \right\} \\
&=& \left[\widehat{\theta} - \gamma, \widehat{\theta} + \gamma \right].
\end{eqnarray*}
Since $\mu( \cdot)$ is the Lebesgue measure, $\mu(\mathcal{C}^{\star}_{\delta}(\widehat{\theta})) = 2 \gamma$.  By Theorem \ref{thm:general}, this confidence region has minimal average (averaged over possible values of $\theta$) among confidence regions satisfying the prescribed coverage. 
\end{ex}

